On Determinism and Unambiguity of Weighted Two-way Automata

In this paper, we first study the conversion of weighted two-way automata to one-way automata. We show that this conversion preserves the unambiguity but does not preserve the determinism. Yet, we prove that the conversion of an unambiguous weighted one-way automaton into a two-way automaton leads to a deterministic two-way automaton. As a consequence, we prove that unambiguous weighted two-way automata are equivalent to deterministic weighted two-way automata in commutative semirings.

==> Dessins/onewayp.tex <==
\VCDraw{%
\begin{VCPicture}{(-1,-2)(6,7)}
\State[p]{(0,5)}{1}
\State[q]{(5,5)}{2}
\ChgStateLabelScale{.85}
\StateVVar[\StackThreeLabels psq]{(0,0)}{3}
\StateVVar[\StackThreeLabels qrp]{(5,0)}{4}
\Initial{1} \Initial{3} \Final[sw]{1} \Final[s]{4}
\LoopN[.5]{1}{b\mid 0} \ArcL[.5] 12{a\mid 0} \ArcL[.5] 21{a\mid 0} \EdgeL[.5] 13{b\mid 0}
\ArcL[.5] 34{a\mid 1}\ArcL[.5] 43{a\mid 1} \EdgeR 41{b\mid 0}
\end{VCPicture}}


==> Dessins/onewayq.tex <==
\VCDraw{%
\begin{VCPicture}{(-6,-4)(11,7)}
\State[p]{(0,5)}{1}
\State[q_+]{(5,5)}{2}
\ChgStateLabelScale{.85}
\StateVVar[\StackThreeLabels p{s_+}{q_+}]{(0,0)}{3}
\StateVVar[\StackThreeLabels p{s_-}{q_+}]{(10,-2)}{3b}
\StateVVar[\StackThreeLabels {q_+}rp]{(5,0)}{4}
\StateVVar[\StackThreeLabels {q_-}rp]{(-5,-2)}{4b}
\Initial{1} \Initial[s]{3} \Final[se]{1} \Final[s]{4b}
\LoopN[.5]{1}{b\mid 0} \ArcL[.5] 12{a\mid 0} \ArcL[.5] 21{a\mid 0} \EdgeL[.5] 13{b\mid 0}
\EdgeL[.5] 34{a\mid 1}\ArcR[.5] 3{4b}{a\mid 1}\ArcR[.5] {4b}3{b\mid 0}\ArcL[.5] 4{3b}{a\mid 1}\ArcL[.5] {3b}4{a\mid 1}\ArcL[.5] {3b}{4b}{a\mid 1} \ArcL {4b}1{b\mid 0}
\end{VCPicture}}


==> Dessins/path.tex <==
\VCDraw{%
\begin{VCPicture}{(-10,-1)(-,1)}
\Point{(-8,0)}{A0}
\Point{(-4,0)}{A1}
\Point{(0,0)}{A2}
\Point{(4,0)}{A3}
\ChgStateLabelScale{.7}
\StateVar[X_0,Y_0]{(-6,0)}{P0}
\StateVar[X_1,Y_1]{(-2,0)}{P1}
%\StateVar[X_2,Y_2]{(2,0)}{P2}
\StateVar[X_k,Y_k]{(6,0)}{P3}
\State{(-10,0)}{PI}
\Initial{PI}\Final{P3}
\EdgeL{A0}{P0}{\ltype}
\EdgeL{A1}{P1}{w_1}
\EdgeL{A3}{P3}{w_k}
\SetEdgeLineStyle{dotted}
\SetEdgeArrowStyle{-}
\EdgeL{PI}{A0}{}
\EdgeL{P0}{A1}{}
\EdgeL{P1}{A2}{}
\EdgeL{A2}{A3}{}
\end{VCPicture}}


==> Dessins/runabaaba.tex <==
\VCDraw[10]{\begin{VCPicture}{(0,0)(2,1.1)}

\psline{-}(0.20,1)(1.8,1)

\multido{\ni=0.2+0.2}{9}{%
\psline{-}(\ni,1.)(\ni,1.05)%
}

\rput(0.3,1.05){\VaucEdgeLabel{\ltype}}
\rput(0.5,1.05){\VaucEdgeLabel{a}}
\rput(0.7,1.05){\VaucEdgeLabel{b}}
\rput(0.9,1.05){\VaucEdgeLabel{a}}
\rput(1.1,1.05){\VaucEdgeLabel{a}}
\rput(1.3,1.05){\VaucEdgeLabel{b}}
\rput(1.5,1.05){\VaucEdgeLabel{a}}
\rput(1.7,1.05){\VaucEdgeLabel{\rtype}}

%\SmallState
\ChgEdgeLabelScale{.8}
%\ChgStateLabelScale{.6}
\State[p]{(0.4,0.9)}{P1}
\State[q]{(0.6,0.9)}{Q1}
\State[r]{(0.6,0.7)}{R1}
\State[s]{(0.4,0.7)}{S1}
\State[q]{(0.4,0.5)}{Q2}
\State[p]{(0.6,0.5)}{P2}
\State[p]{(0.8,0.5)}{P3}
\State[q]{(1.0,0.5)}{Q3}
\State[p]{(1.2,0.5)}{P4}
\State[p]{(1.4,0.5)}{P5}
\State[q]{(1.6,0.5)}{Q5}
\State[r]{(1.6,0.3)}{R5}
\State[s]{(1.4,0.3)}{S5}
\State[q]{(1.4,0.1)}{Q6}
\State[p]{(1.6,0.1)}{P6}
\Initial{P1}
\EdgeL{P1}{Q1}{\rightarrow|0}
\VArcL[.2]{arcangle=70,ncurv=1.2}{Q1}{R1}{\leftarrow|0}
\EdgeR{R1}{S1}{\leftarrow|1}
\VArcR[.2]{arcangle=-70,ncurv=1.2}{S1}{Q2}{\rightarrow|0}
\EdgeL{Q2}{P2}{\rightarrow|0}
\EdgeL{P2}{P3}{\rightarrow|0}
\EdgeL{P3}{Q3}{\rightarrow|0}
\EdgeL{Q3}{P4}{\rightarrow|0}
\EdgeL{P4}{P5}{\rightarrow|0}
\EdgeL{P5}{Q5}{\rightarrow|0}
\VArcL[.2]{arcangle=70,ncurv=1.2}{Q5}{R5}{\leftarrow|0}
\EdgeR{R5}{S5}{\leftarrow|1}
\VArcR[.2]{arcangle=-70,ncurv=1.2}{S5}{Q6}{\rightarrow|0}
\EdgeL{Q6}{P6}{\rightarrow|0}
\Final{P6}

\end{VCPicture}}


==> Dessins/twoway.tex <==
\VCDraw{\begin{VCPicture}{(-2,-4)(20,3)}
\State[p]{(0,0)}{1}
\State[q]{(6,0)}{2}
\State[r]{(12,0)}{3}
\State[s]{(18,0)}{4}
\Initial 1 \Final[s]1
\LoopN[.5] 1{b,\rightarrow\mid 0} \ArcL[.5] 12{a,\rightarrow\mid 0} \ArcL[.5] 21{a,\rightarrow\mid 0} \EdgeL[.5] 23{\StackTwoLabels{\rtype,\leftarrow\mid 0}{b,\leftarrow\mid 0}}
\ArcL[.5] 34{a,\leftarrow\mid 1} \ArcL[.5] 43{a,\leftarrow\mid 1} \VArcL[.5]{arcangle=90,ncurv=.3} 42{\StackTwoLabels{b,\rightarrow\mid 0}{\ltype,\rightarrow\mid 0}}
\end{VCPicture}}


==> Dessins/twowayd.tex <==
\VCDraw{%
\begin{VCPicture}{(-2,-4)(20,3)}
\State[p]{(0,0)}{1}
\State[q]{(6,0)}{2}
\State[r]{(12,0)}{3}
\State[s_-]{(18,1)}{4}
\State[s_+]{(18,-1)}{5}
\Initial 1 \Final[s]1
\LoopN[.5] 1{b,\rightarrow\mid 0} \ArcL[.5] 12{a,\rightarrow\mid 0} \ArcL[.5] 21{a,\rightarrow\mid 0} \EdgeL[.5] 23{\StackTwoLabels{\rtype,\leftarrow\mid 0}{b,\leftarrow\mid 0}}
\ArcL[.5] 34{a,\leftarrow\mid 1}\ArcR[.5] 35{a,\leftarrow\mid 1} \ArcL[.5] 43{a,\leftarrow\mid 1}
\VArcL[.5]{arcangle=90,ncurv=.3} 52{\StackTwoLabels{b,\rightarrow\mid 0}{\ltype,\rightarrow\mid 0}}
\end{VCPicture}}


==> Dessins/twowayp.tex <==
\VCDraw{\begin{VCPicture}{(-2,-2)(14,3)}
\State[p]{(0,0)}{1}
\State[q]{(6,0)}{2}
\State[r]{(12,0)}{3}
\Initial 1 \Final[ne]2
\LoopN[.5] 1{\StackTwoLabels{0,\rightarrow\mid 1/2}{1,\rightarrow\mid 1/2}} \EdgeL[.5] 12{1,\rightarrow\mid \frac 12}
\LoopN[.5] 2{\StackTwoLabels{0,\rightarrow\mid 1}{1,\rightarrow\mid 1}}
\LoopN[.5] 3{\StackTwoLabels{0,\leftarrow\mid 1}{1,\leftarrow\mid 1}}
\EdgeL[.5] 23{\rtype,\leftarrow\mid 1}
\ArcL 31{\ltype,\rightarrow\mid 1}
\end{VCPicture}}


==> Dessins/unamb-det.tex <==
\FixVCScale{.52}
\VCDraw{%
\begin{VCPicture}{(-4.5,-13)(17,12)}
\State[i]{(17,6)}{i}
\Initial i
\LoopN[.5]i{\StackTwoLabels{a,\rightarrow}{b,\rightarrow}}
\LargeState
\ChgStateLabelScale{.8}
\State[\StackTwoLabels{1}{4}]{(17,2)}{T}
\State[\StackTwoLabels{2}{3}]{(17,-1)}{U}
\EdgeL iT{\rtype,\leftarrow}
\LoopE T{b,\leftarrow}
\ArcL TU{a,\leftarrow}
\ArcL UT{\StackTwoLabels{a,\leftarrow}{b,\leftarrow}}
\StateVar[\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(7,5)}{IT}
\EdgeR[.6]T{IT}{\ltype,\rightarrow|0}
\FinalL{e}{IT}{|0}
\StateVar[a,1,\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(11,7)}{aIT}
\EdgeL{IT}{aIT}{a,\rightarrow}
\StateVar[\alpha,1,\StackTwoLabels{1}{3},\StackTwoLabels{2}{3}]{(11,10)}{raIU}
\EdgeR{aIT}{raIU}{\StackTwoLabels{a,\leftarrow}{\color{lightgray}b,\leftarrow}}
\StateVar[\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(7,12)}{JU}
\EdgeR{raIU}{JU}{a,\rightarrow|0}
\StateVar[a,1,\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(3,10)}{aJU}
\EdgeR{JU}{aJU}{a,\rightarrow}
\StateVar[\alpha,1,\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(3,7)}{raJT}
\EdgeR{aJU}{raJT}{\StackThreeLabels{a,\leftarrow}{b,\leftarrow}{\rtype,\leftarrow}}
\EdgeL{raJT}{IT}{a,\rightarrow|0}
\StateVar[b,1,\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(7,2)}{bIT}
\EdgeL{IT}{bIT}{b,\rightarrow}
\StateVar[\beta,1,\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(2,2)}{rbIT}
\StateVar[\beta,\alpha,\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(2,-1)}{rbalIT}
\EdgeL{bIT}{rbIT}{\StackTwoLabels{b,\leftarrow}{\rtype,\leftarrow}}
\EdgeL{rbIT}{IT}{b,\rightarrow|0}
\ArcL{rbIT}{rbalIT}{a,\leftarrow}
\ArcL{rbalIT}{rbIT}{a,\leftarrow}
\StateVar[b,\alpha,\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(12,2)}{balIT}
\ArcL{bIT}{balIT}{a,\rightarrow}
\ArcL{balIT}{bIT}{a,\rightarrow}
\StateVar[\beta\alpha,1,\StackTwoLabels{1}{3},\StackTwoLabels{2}{3}]{(12,-1)}{baIU}
\EdgeL{balIT}{baIU}{b,\leftarrow}
\StateVar[\beta\alpha,\alpha,\StackTwoLabels{1}{3},\StackTwoLabels{2}{3}]{(7,-1)}{baalIU}
\ArcL{baIU}{baalIU}{a,\leftarrow}
\ArcL{baalIU}{baIU}{a,\leftarrow}
\StateVar[\StackTwoLabels{1}{3},\StackTwoLabels{2}{3}]{(7,-4)}{IU}
\EdgeL U{IU}{\ltype,\rightarrow|0}
\EdgeL{baalIU}{IU}{b,\rightarrow|0}
\StateVar[a,1,\StackTwoLabels{1}{3},\StackTwoLabels{2}{3}]{(11,-6)}{aIU}
\EdgeL{IU}{aIU}{a,\rightarrow}
\StateVar[\alpha,1,\StackTwoLabels{1}{3},\StackTwoLabels{1}{4}]{(11,-9)}{raIT}
\EdgeR{aIU}{raIT}{\StackThreeLabels{a,\leftarrow}{b,\leftarrow}{\rtype,\leftarrow}}
\StateVar[\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(7,-11)}{JT}
\FinalL{s}{JT}{|0}
\EdgeL{raIT}{JT}{a,\rightarrow|1}
\StateVar[a,1,\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(3,-9)}{aJT}
\EdgeL{JT}{aJT}{a,\rightarrow}
\StateVar[\alpha,1,\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(3,-6)}{raJU}
\EdgeR{aJT}{raJU}{\StackTwoLabels{a,\leftarrow}{\color{lightgray}b,\leftarrow}}
\EdgeL{raJU}{IU}{a,\rightarrow|1}
\StateVar[b,1,\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(-3,-9)}{bJT}
\ArcL{JT}{bJT}{b,\rightarrow}
\StateVar[\beta,1,\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(-3,2)}{rbJT}
\VArcL{arcangle=50}{bJT}{rbJT}{\StackTwoLabels{b,\leftarrow}{\rtype,\leftarrow}}
\ArcL[.3]{rbJT}{IT}{b,\rightarrow|0}
\StateVar[\beta,\alpha,\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(-3,-1)}{rbalJT}
\ArcL{rbJT}{rbalJT}{a,\leftarrow}
\ArcL{rbalJT}{rbJT}{a,\leftarrow}
\StateVar[b,\alpha,\StackTwoLabels{2}{4},\StackTwoLabels{1}{4}]{(-3,-6)}{balJT}
\ArcL[.6]{bJT}{balJT}{a,\rightarrow}
\ArcL{balJT}{bJT}{a,\rightarrow}
\StateVar[\beta\alpha,1,\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(-3,-3)}{rbaJU}
\EdgeL{balJT}{rbaJU}{b,\leftarrow}
\StateVar[\beta\alpha,\alpha,\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(2,-3)}{rbaalJU}
\ArcL[.3]{rbaJU}{rbaalJU}{a,\leftarrow}
\ArcL[.7]{rbaalJU}{rbaJU}{a,\leftarrow}
\EdgeL{rbaalJU}{IU}{b,\rightarrow|0}
\ChgStateLineColor{lightgray}
\ChgStateLabelColor{lightgray}
\ChgEdgeLineColor{lightgray}
\ChgEdgeLabelColor{lightgray}
\VArcL[.9]{arcangle=40}{aIT}{raIT}{\rtype,\leftarrow}
\VArcL[.1]{arcangle=40}{aJT}{raJT}{\rtype,\leftarrow}
\StateVar[b,1,\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(7,8.5)}{bJU}
\EdgeL{JU}{bJU}{b,\rightarrow}
%\ArcR{bJU}{rbJT}{\StackTwoLabels{b,\leftarrow}{\rtype,\leftarrow}}
%\StateVar[b,\alpha,\StackTwoLabels{2}{4},\StackTwoLabels{2}{3}]{(17,-13)}{balJU}
%\ArcR{bJU}{balJU}{a,\rightarrow}
%\ArcR{balJU}{bJU}{a,\rightarrow}
\StateVar[b,1,\StackTwoLabels{1}{3},\StackTwoLabels{2}{3}]{(7,-7.5)}{bIU}
\EdgeL{IU}{bIU}{b,\rightarrow}
\end{VCPicture}}


==> eptcsdata.tex <==
\providecommand{\firstpage}{188}
\providecommand{\publicationstatus}{Z. \'Esik and Z. F\"ul\"op (Eds.): Automata and Formal Languages 2014 (AFL 2014)\\
EPTCS 151, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.151.13}{10.4204/EPTCS.151.13}}

